Framework and Tools for the Simulation and Analysis of the Radio Emission from Air Showers at IceCube

The Surface Enhancement of the IceTop air-shower array will include the addition of radio antennas and scintillator panels, co-located with the existing ice-Cherenkov tanks and covering an area of about 1 km$^2$. Together, these will increase the sensitivity of the IceCube Neutrino Observatory to the electromagnetic and muonic components of cosmic-ray-induced air showers at the South Pole. The inclusion of the radio technique necessitates an expanded set of simulation and analysis tools to explore the radio-frequency emission from air showers in the 70 MHz to 350 MHz band. In this paper we describe the software modules that have been developed to work with time- and frequency-domain information within IceCube's existing software framework, IceTray, which is used by the entire IceCube collaboration. The software includes a method by which air-shower simulation, generated using CoREAS, can be reused via waveform interpolation, thus overcoming a significant computational hurdle in the field.

==> Removed_Section4.tex <==
\section{Frequency Weighting Scheme}
\label{s:freq_weighting}

For an array designed to measure the radio emission from air showers, the limiting factor to which the properties of the cosmic ray can be determined is largely due to the local noise.
The overall noise profile is comprised of both coherent and non-coherent emissions as well as electronic noise from the readout hardware.
At the South Pole, the noise floor is set by the emission from Galactic and extra-Galactic sources and is generally non-coherent.
There are also sources of coherent RFI at the South Pole.
While non-coherent noise sets a minimum primary energy threshold for a given array, coherent noise can cause pulses which are hard to distinguish from those emitted by air showers.
In the second case, the accidental inclusion of RFI pulses decreases the overall accuracy of the reconstruction, regardless of the energy of the cosmic ray.

The median local noise profile at the South Pole has been measured using a prototype station and is shown in blue in \cref{fig:spike_filter}.
%
%
\begin{figure}[t]
\centering
\includegraphics[width=0.8\columnwidth]{figures/SpikeFilter_CRBased.pdf}
\caption{The median power observed by the prototype station at the South Pole using TAXI v3.0 is shown in blue. This, combined with the average cosmic ray spectrum (yellow) were used to develop a frequency-weighting scheme (red). A model of the average Galactic noise at the South Pole is shown in dashed black. The bottom panel shows the frequency weights, see \cref{eq:weighting_scheme}.}
\label{fig:spike_filter}
\end{figure}
%
%
The expected emission from Galactic and extra-Galactic sources has been determined using the Cane model~\cite{cane1979spectra} and the thermal noise has been modeled using an effective temperature of 30\,K and is shown via the dashed black line in the same figure.
While there is a band, $\simeq$\,100 to 250\,MHz, on which the noise levels are approximately at about the minimum expected levels, there are several RFI peaks at, for instance, 250 and 280\,MHz.
There is also broadband noise for frequencies below $\simeq 100$\,MHz.\footnote{This broadband noise has been identified as coming from TAXI itself and will be mitigated in the version that will be deployed on the full-scale array.}

One common method for reducing narrow-band noise is to apply a median filter to the individual waveforms.
In this method, the amplitudes of the frequency spectrum, $a_i$, are replaced by the median value in a window with half-width, $h$,
\begin{equation}
    a_i' = {\rm Median}(\{a_{i - h},\, ...,\, a_{i+h}\}).
    \label{eq:median_filter}
\end{equation}
A second method is to apply notch filters, either in the analysis or directly in the hardware, wherein the amplitudes in specific frequency bands are removed.

In this section, we describe the effectiveness of an alternative method which builds on these two techniques.
In \cref{ss:dev_filter}, we detail how we construct a set of weights for each frequency bin which inherently applies the notching technique but without the need to choose the bands by hand.
We verify the impact of this method via a calculation of the reconstruction efficiency of the array, using simulations with measured noise in \cref{ss:filter_poc}.


\subsection{Development of the Filter}
\label{ss:dev_filter}

The frequency weighting scheme combines the observed background pulses with the frequency spectrum of air shower radio emission.
For this purpose, we created a second library of air shower simulations.
At the South Pole, the local geomagnetic field is 17.8\degr from the zenith and is 30.7\degr west of grid north.
Because the strength of the geomagnetic emission process depends on the angle with the local magnetic field, we simulated directions which spanned the full range of geomagnetic angles.
Equally spaced zenith angles were chosen, 0\degr, 17\degr, 34\degr, 51\degr, and 68\degr, and azimuth angles of 30.7\degr west-of-north and east-of-south used. 
Discrete energy bins from 10 to 1000\,PeV were used, equally spaced in $\lg (E/{\rm eV})$.
Both proton and iron primaries were used and for each zenith/azimuth/energy/primary bin, 200 cascades were simulated.
Otherwise, all CORSIKA settings are the same as described in \cref{ss:SimOnStar}.
The electric field waveforms were then propagated through the end-to-end simulation chain described in \cref{ss:end_to_end_sim}.

To calculate the weights for each frequency bin, we used the bin-wise median values, $m_i$, of the local background at the South Pole, as shown in blue in \cref{fig:spike_filter}.
We then used the voltages, folded with the detector response, from the library of air-shower simulations, using only the pure signal, with no noise added.
We calculated the average power spectrum, $\mathcal{C}_i$, of air showers with a primary energy of 300\,PeV, using only the three antennas in each event for which the Hilbert envelope was the largest.
Finally, we constructed the weights, $w_i$, using the ratio of these two values,
\begin{equation}
    w_i = \mathcal{N}(\mathcal{C}_i/m_i)^2.
    \label{eq:weighting_scheme}
\end{equation}
Here, $\mathcal{N}$ is a normalization such that the largest value of $w_i$ is unity.

The average cosmic ray power spectrum is shown in gold in \cref{fig:spike_filter} while the background noise with the applied weights, $w_i \times m_i$, is shown in red.
The bottom portion of the figure, directly shows the value of $\mathcal{C}_i/m_i$.
The result is that the RFI peaks become a similarly deep valley, penalizing all features which are less smooth than, $\mathcal{C}_i$.
Additionally, this process simultaneously accentuates the frequency bands where $\mathcal{C}_i$ is harder than $m_i$, as seen in the larger overall values of the weights for 100 to 200\,MHz as compared to 200 to 350\,MHz.


\subsection{Comparison to a Median Filter}
\label{ss:filter_poc}

As a proof of concept, we then compared this frequency weighting scheme to one of the common methods for removing RFI-peaks, namely, the median filter (\cref{eq:median_filter}).
As a metric by which to compare, we calculate the reconstruction efficiency of air showers using the antenna array for the two methods.
This is motivated by the fact that if there are high-amplitude RFI pulses in the waveforms, a proportionally high threshold must be required to reject these pulses, thus raising the energy threshold for cosmic ray detection.

To determine which waveforms to keep for a given event, we used a criteria based on the signal-to-noise ratio (SNR) of the power, $P$,
\begin{equation}
    {\rm SNR} = \frac{P_{\rm Signal}}{P_{\rm Noise}} = \left( \frac{\rm HilbertPeak}{\rm RMS} \right)^2.
\end{equation}
The peak of the Hilbert envelope and the RMS voltage were calculated in separate windows so as to reduce the influence of the true signal on the estimation of the noise.
We used non-overlapping signal and noise windows of length 200\,ns and 400\,ns, respectively.
The width of the signal window is motivated by the $\leq 1^\circ$ angular resolution of the scintillator array, which provides the external trigger and therefore a reconstructed axis~\cite{Leszczynska:2019ahq}.
An example background waveform with ${\rm SNR} = 45.7$ is shown in the top plot of \cref{fig:snr_optimal} along with the signal and noise windows.
%
%
\begin{figure}[t]
\centering
\includegraphics[width=0.7\columnwidth]{figures/ExampleWaveform_SNR45.7.pdf}\\
\vspace{0.5cm}
\includegraphics[width=0.42\columnwidth]{figures/SNRAnalysis_CutValues_CR_Pow2.pdf}
\qquad
\includegraphics[width=0.42\columnwidth]{figures/OptimalBand_CR_Pow2.pdf}
\caption{Top: A pure-background waveform, measured using TAXI v3.0, which has an SNR value of 45.7. The signal and noise windows used to calculated the SNR are shown in dashed blue and dotted red, respectively. Bottom left: A scan of the SNR threshold corresponding to a background waveform rejection of 99\% is shown as a function of the upper and lower edge of the band being used. Bottom right: The average number of antennas per shower with ${\rm SNR} > \hat{S}_{99}$ for simulated air showers with measured noise added. The optimal band, given by the maximum value, is indicated by the black dot (corresponding to an SNR cut of 45.7).}
\label{fig:snr_optimal}
\end{figure}
%
%

To determine the SNR cut threshold for the two RFI-filtering schemes, 30k background waveforms were analyzed with randomly placed signal and noise windows.
We then applied a band-pass filter to each of the waveforms, scanning in the lower and upper frequency band limit, $f_{\rm low}$ and $f_{\rm high}$, respectively, on which to apply the band.
The SNR-cut value which rejects 99\% of background pulses in the various bands, $\hat{S}_{99}(f_{\rm low},f_{\rm high})$, are shown in the lower left plot of \cref{fig:snr_optimal} for the frequency weighting scheme.

Finally, we determined the optimal band on which to most readily identify cosmic ray air showers given the set of $\hat{S}_{99}(f_{\rm low},f_{\rm high})$.
In this process, we added measured noise, recorded at the South Pole, to the simulated voltages of the 96 antennas in the array and applied one of the two relevant RFI filters.
Again, a series of band-pass filters were applied and the corresponding SNR values were checked against the corresponding cut.
The optimal band was then chosen to be the one for which there were the most number of antennas with ${\rm SNR} > \hat{S}_{99}(f_{\rm low},f_{\rm high})$.

To reduce the impact of choosing a frequency band that is only appropriate for a subset of the overall phase space, this process was first conducted only on 300\,PeV air showers.
The optimal band and corresponding SNR cut was determined and then the reconstruction efficiency was calculated (described below).
This process was then repeated using only the showers with energy and direction for which the reconstruction efficiency is between 30\% and 70\%.
The average number of antennas which pass the corresponding SNR cut per event for the frequency weighting scheme is shown in the bottom right plot of \cref{fig:snr_optimal}.
The optimal band of 110 to 190\,MHz is indicated by the black dot.

Finally, we determined the reconstruction efficiency of the radio array.
An event is considered successfully reconstructed if the arrival direction of the air shower, as determined using a plane wave fit to the Hilbert peak times, is within 5$^\circ$ of the true value.
The efficiency of the array for iron and proton primaries are shown separately for the RFI-reduction methods in \cref{fig:det_eff}.
%
%
\begin{figure*}[t]
\centering
\includegraphics[width=0.45\columnwidth]{figures/DetectionEfficiency_CR_pow2_105-190MHz_prot.pdf}
\includegraphics[width=0.45\columnwidth]{figures/DetectionEfficiency_CR_pow2_105-190MHz_iron.pdf}\\
\vspace{0.5cm}
\includegraphics[width=0.45\columnwidth]{figures/DetectionEfficiency_Median-31bins-120_185MHz-proton.pdf}
\includegraphics[width=0.45\columnwidth]{figures/DetectionEfficiency_Median-31bins-120_185MHz-iron.pdf}
\caption{The reconstruction efficiency of the array is compared for simulated proton (left) and iron (right) primaries. The top plots show the efficiency using the frequency weighting scheme shown in \cref{fig:spike_filter} while the bottom plots are for a median filter with a 31 MHz width. A reconstruction is deemed successful if a plane wave fit agrees to within $5^\circ$ of the Monte-Carlo truth.}
\label{fig:det_eff}
\end{figure*}
%
%
The top plots correspond to the frequency weighting scheme while the bottom plots correspond to the median filter.
The frequency weighting scheme shows a strict improvement over that of the median window by about 10\% (see \ref{app:efficiency_improvement} for a more detailed comparison).
Since the frequency weighting scheme both removes RFI peaks as well as generally rescale the overall slope of each waveform's frequency spectrum, it is unclear which of these is more important.

This method can be further extended in various ways.
Firstly, the median background spectrum, $m_i$, was calculated using all of the background waveforms in all antennas, together.
However, in practice, each arm of the antenna will have a different orientation to the source(s) of RFI and galactic noise.
One could thus instead calculate a set of weights on a per-antenna, or even per-channel basis.
Secondly, the distribution of waveforms used when calculating the average frequency spectrum from air showers could be chosen differently.
Instead of using the three per event with the largest true-signal peak, one could instead use antennas which are off of the Cherenkov ring and thus harder to detect in the first place.
Further, one could use only a subset of the phase space of simulated showers considered so as to increase the detection efficiency for, say, only vertical air showers.
Regardless, even without these potential optimizations, this study demonstrates that this method of re-weighting individual frequencies is as-good if not better for the rejection of background pulses and subsequent identification of air showers.
